Structural Generalization in Autonomous Cyber Incident Response with Message-Passing Neural Networks and Reinforcement Learning

We believe that agents for automated incident response based on machine learning need to handle changes in network structure. Computer networks are dynamic, and can naturally change in structure over time. Retraining agents for small network changes costs time and energy. We attempt to address this issue with an existing method of relational agent learning, where the relations between objects are assumed to remain consistent across problem instances. The state of the computer network is represented as a relational graph and encoded through a message passing neural network. The message passing neural network and an agent policy using the encoding are optimized end-to-end using reinforcement learning. We evaluate the approach on the second instance of the Cyber Autonomy Gym for Experimentation (CAGE~2), a cyber incident simulator that simulates attacks on an enterprise network. We create variants of the original network with different numbers of hosts and agents are tested without additional training on them. Our results show that agents using relational information are able to find solutions despite changes to the network, and can perform optimally in some instances. Agents using the default vector state representation perform better, but need to be specially trained on each network variant, demonstrating a trade-off between specialization and generalization.

==> scratchpad.tex <==
\subsection{Problem Description}
\label{sec:problem}
Our problem definition. 

Relational reinforcement learning.

First order Markov decision process.

Factored Markov decision process.

Object-oriented reinforcement learning.

%Decision problems where the input space is either a set or a graph.

We assume the domain to be finite.

%The method should be invariant or equivariant to
%changes in the input. For example, if the same entity appears in a different
%part of the input, the agent should treat it as the same entity as before.

% \textcite{janisch2023symbolic} demonstrates the problem in three environments. 


\subsection{Applicability to computer networks}

Do's and don'ts \cite{dodos}.

There are not really any physical limitations to the number of actions an agent
can take in their turn. The formulation used by \textcite{janisch2023symbolic}
can be modified to allow the agnet to actions on multiple objects inthe same
turn. Active responses in Wazuh can take any number of objects as a parameter.

Multiple actions can also be intrepreted as a multi-agent environment. Each
agent is an object in the network.

We find it somewhat peculiar that any solution that explicitly includes the
attacker policy would be considered at all usable. The solutions may solve this
particular toy problem, but to claim anything other than that would be a gross
exaggeration.

\subsection{Vulnerability to attacks}

Cyber security is an inherently adversarial context \cite{dodos}. Include the
paper on attacks on graph-based IDS. Adversary stuffing the graph with useless
information. Adversarial policies.

\subsection{Limitations of the CybORG envirionment}


No defined object types. We arguably have two types of objects. Hosts and routers.

We removed the red team starting machine from the action space of the blue team.
We motivate this change by the fact that there is nothing apart from the host index 
in the wrapped observation space that
indicates that this host is different from the rest, despite 
following different rules. Remove and restore actions on the machine the attacker
starts at are guaranteed to fail. Given that we would like our agent to not
learn dynamics that are bound to a particular host, we opt for simply removing
the host from the action space. To get ahead of anyone objecting this change, we
will to note that the team responsible for the top entry of the leader-board
also made this change.

Hosts are mapped to specific indices in the vector, the position of a host in
the vector is a unique identifier for that host. For a neural network, this
means that a.

CybORG is arguably one of the more realistic cyber-incident simulators in the
current of simulators. It can provides information that resembles the data that
would be obtained from an actual computer network monitoring tool. It allows
training both offensive and defensive agents, both individually and at the same
time. Being able to train both offensive and defensive agents in the same
environment is useful when learning through self-play or analyzing adversarial
attacks against \ac{rl}-based systems.

The wrapper used for the CAGE challenge strips the environment of some of these
benefits however. It adds a set of heuristics that will inform if a host has
been compromised. The developers themselves note that the information provided
in the wrapper is unrealistic. Though the green agent is intended to introduce
some degree of difficulty here, it is not used in any of the official evaluation
scripts..

The effects of agent actions are better represented in the unwrapped observation
space. If a decoy is deployed, it will show up as a process in the list. If a
scan is successful, new information is added to the data structure. However,
this data structure is highly heterogeneous. Utilizing the unwrapped
observations is an interesting venue for future work in our opinion.

We do not use decoy actions. To successfully deploy a decoy process in CybORG 
an agent needs information about the operating system, ports and processes on a particular host. 
This is not present in the wrapped observation space other than the index, i.e. name of
a host. There does exist an abstract action in the set of possible actions,
named \enquote{misinform}, that will automatically select a random compatible
decoy. The problem remains still that the decoy is not represented in the state
space, and the agent can therefore not know that it is deployed.

We believe that effective deployment of decoy processes requires information
about hosts not present in the wrapped observation space. As stated in
\ref{sec:cyborg}. When hosts are encoded in fixed positions in a vector, the
policy can rely on this information when selecting a decoy.

We ultimately opted to not using decoys as our goal was not to optimize decoy
deployment, and the resulting policies work fine without them. We recognize,
however, that we are unlikely to reach the same levels of reward as previous
work due to this change as the deployment of decoys are beneficial to the blue
team task.


In writing this paper we were conflicted on whether to address these issues, or
take the problem at face value. Extensive modification of the environment would
make it more difficult for us to compare to previous work. Previous work is
unlikely to have done so. None of the previous work that we have observed has
analyzed the trained policies in any detail. \cite{wolk2022cage} includes a
histogram showing the distribution of agent actions.

There is no negative reward for performing the remove action. An agent can
therefore get a decent score by repeating it. We do not consider this desirable
behavior in an incident response agent, as this behavior would cause disruptions
in real life.

The term \enquote{simulator} may be somewhat generous, as it brings to mind
models based in physical reality, built upon established models of reality. The
simulators of cyber environments tend to operate on a high level of abstraction,
loosely inspired by reality. Cyber incident games may be a more accurate moniker
for most of them.

The documentation around the cyborg environment differs from the code
implementation. Seven decoy actions are listed in the documentation for the
second challenge, though eight are actually provided in the code. Written
correspondence with one of the authors has informed us that the eight decoy
will not have any effect in scenario 2, and is functionally a null action.

\ac{cyborg} has a green agent. The green agent is intended to simulate user
activity. In practice, this means that the agent is performing port scans.
These show up as scanning activity for the defender. The green agent is
described in the documentation, but is not used in the script used for
evaluating agents. None of the implementations we have found has incorporated
the green agent in training or evaluation, despite some mentioning it in their
descriptions of \ac{cyborg} and \ac{cage}. As far as our understanding goes,
this implies that there are no false positives in the \enquote{standard}
configuration of scenario 2.

This has been propagated in later work, such as \cite{wolk2022cage}. The sleep
action is not listed on the Github page. The monitor action is redundant for
the blue agent, as it is always executed regardless of what action is taken.

\subsection{Other generalizations}

We focus generalization over network topologies 
as the only form 

There are, however, other sources of variability that may be desirable 
to handle. Policy functions are optimal given a reward function. If the reward function
changes the policy may have to change in order to remain optimal. Our
assumption here is therefore that the reward function does not
significantly change when the number of objects change. 

Meta-reinforcement learning. Attacker behavior that would change the
relative values of states. This has also been noted by
\textcite{wolk2022cage}.  Of interest to us is how to problem may be
solved independent of the number of objects. Other forms of
meta-learning could perhaps be used to address other sources of
variability.


The model architecture can in theory handle the state changing in size during training. 
We do not test this.

\subsection{Graph Learning}

Evolving graph. We limited ourselves in this work to a graph that remains static
over the course of an episode. The is partially an implementation issue.
Handling efficient batching of graph-structured data is not something the common
RL frameworks support.

Can the \ac{gnn} represent the states uniquely? A stochastic policy can handle
ambiguous representations, but it risks hurting policy performance. If we use an
MLP, or encode a graph representation, all state representations are unique. The
graph neural network may encode two different nodes using the same
representation. If the latter choice is made only based on the ndoe embedding it
may be impossible to act optimally. the weishfehler lehman. how expressie are
gnn. higher order weisfehler lehman.

Can be tested using imitation learning. Optimize the MLP to the optimal policy
and then train the \ac{gnn}. If the \ac{gnn}-based policy can not encode the
optimal policy there is something wrong with the representations.

Value function prediction is required during training if an actor-critic method
is used. The value function is not needed during policy evaluation, so if the
policy function does not depend on global state then we only depend on local
sub-trees.

There exist a number of modifications
that could be made to the \ac{gnn} architecture~\cite{designspace}. As we are
not overly interested in chasing high-scores, and the high variance of the
environment make qualitative comparisons difficult, we did not extensively study
these modifications.

Extended by \textcite{oracle-sage} in their approach named Oracle-SAGE, which
combines a planning component from the authors previous work, SAGE, with SR-DRL.
\textcite{oracle-sage} addresses the limitation of the information-horizon that the message-passing introduces.


\subsection{Topology Generalization}

Convolutional neural networks. \acp{cnn} do not scale the amount of parameters with the input. 
However, \acp{cnn} are not permutation invariant or equivariant.

\acp{cnn} and transformers are arguably less general forms of \acp{gnn}. 
A transformer is permutation invariant, and equivariant, but assumes 
that the input is a fully connected graph.

A CNN uses a fixed node ordering, and is not permutation invariant.


One way of generalizing across topologies is to ignore the topology altogether.
Aggregating alert types across different hosts. Then we are locked to a fixed set
of alerts instead.

The issue of the model being locked to specific positions occurs at
two places in the architecture, the embedding of the state space and
the policy network. \acp{mlp} can not handle changes to input order or
size, as the model weights are associated to positions in the input
vector.

Fine tuning is an option in some cases. The ideal is zero-shot
performance, where the model can operate optimally in an unseen
environment without additional training. Few-shot training and
transfer learning. Networks change.

Another issue is that MLP-based architectures are locked to a fixed
input size, and changes to the size requires that at least parts of
the model are retrained.

Retraining, or applying transfer learning, is an option. Having to
retraining models from scratch is expensive.

The issues of MLP's being input invariant are not unique to this
domain. Within image recognition, 
convolutional neural networks are invariant to input size and translation.

Recurrent neural networks impose an order on the input.
Transformers can handle variable input lengths, 
and are arguably a form of graph neural network, but their complexity
increases exponentially with input size.

We choose to focus on graph neural networks are also
invariant. Computer networks can be modeled as graphs.

However, this by itself is not enough, as we also want the actions to be equivariant, meaning that a permutation of the nodes should cause the same permutation for actions. 
If we were to embed the graph to a vector, and take actions based on that, this requirement would not be fulfilled.

\subsection{Other Simulators}

The third CAGE-challenge deals with a drone network. This can naturally be
represented as a graph, with the drones as node and the distances between them
as edges. Multi-agent reinforcement learning.

CyberBattlesim. Developed by Microsoft. Highly abstracted. Does not support
defensive actions in the original implementation. Extended by subsequent works,
such as \cite{10216719} or \cite{applebaumtabular} to allow training defensive
agents.
